Robust and Performance Incentivizing Algorithms for Multi-Armed Bandits with Strategic Agents

Motivated by applications such as online labor markets we consider a variant of the stochastic multi-armed bandit problem where we have a collection of arms representing strategic agents with different performance characteristics. The platform (principal) chooses an agent in each round to complete a task. Unlike the standard setting, when an arm is pulled it can modify its reward by absorbing it or improving it at the expense of a higher cost. The principle has to solve a mechanism design problem to incentivize the arms to give their best performance. However, since even with an effective mechanism agents may still deviate from rational behavior, the principal wants a robust algorithm that also gives a non-vacuous guarantee on the total accumulated rewards under non-equilibrium behavior. In this paper, we introduce a class of bandit algorithms that meet the two objectives of performance incentivization and robustness simultaneously. We do this by identifying a collection of intuitive properties that a bandit algorithm has to satisfy to achieve these objectives. Finally, we show that settings where the principal has no information about the arms' performance characteristics can be handled by combining ideas from second price auctions with our algorithms.

==> NeccesaryAndSufficient.tex <==
\newpage
\section{Necessary and Sufficient Conditions for Best Performance Equilibrium}
\begin{definition}\label{def:strong_apprx_equilibrium}
Strong approximate equilibrium: For mechanism $\mech$,a strategy profile $S$ is a strong approximate equilibrium if given any arm $i$ we have: 
\begin{align}
    & u_i(S'_i, S_{-i}|\mech) = \Omega(n) \ \ \ \forall i \in [k]\\ 
    & u_i(S'_i, S_{-i}|\mech) \leq u_i(S_i, S_{-i}|\mech) + o(n)   \ \ \ \ \ \text{for any other strategy $S'_i$} 
\end{align}
\end{definition}

We now give a simple condition for a sharply robust algorithm to have $\Sbest$ as \emph{strong} approximate equilibrium. 
\begin{definition}\label{def:LPT}
\textbf{Linear Pulls}: For a monotonic MAB algorithm $\alg$, if arms other than $i$ follow $S^*_{-i}$, then $\E[\totpulls{i}(n)|S^*_i,S^*_{-i}] = \lpt n+o(n)$ where $\lpt \in (0,1)$ is a constant dependent on the specific MAB algorithm. 
\end{definition}

\begin{definition}\label{def:monotonic}
\textbf{Relaxed Monotonicity}: For a monotonic MAB algorithm $\alg$, if arms other than $i$ follow $S^*_{-i}$, then for any possible strategy $S_i$ we have $\E[\totpulls{i}(n)|S_i,S^*_{-i}] \leq \E[\totpulls{i}(n)|S^*_i,S^*_{-i}]+ o(n)$. 
\end{definition}

\begin{theorem}
Given a sharply robust algorithm $\alg$ then $\Sbest$ is a strong approximate equilibrium if and only if $\alg$ satisfies linear pulls and relaxed monotonicity.
\end{theorem}
\begin{proof}
We begin by proving sufficiency: 
\begin{lemma}
For a sharply robust algorithm linear pulls and relaxed monotonicity are sufficient to have $\Sbest$ as a strong approximate equilibrium.  
\end{lemma}
We begin by lower bounding the utility of arm $i$ when it follows strategy $S^*_i$ given $S^*_{-i}$:

\begin{claim}
\begin{align}
    u_i(S^*_i,S^*_{-i}) \ge \meani \lpt n - o(n) 
\end{align}
\end{claim}

\begin{proof}
Since the algorithm satisfies linear pulls it follows under strategy profile $S^*$ that $\forall i \in [k]: \E[\totpulls{i}(n)] \ge \lpt n -o(n)$ where $\lpt \in (0,1)$ is dependent on the algorithm, therefore we have: 
\begin{align}
    u_i(S^*_i,S^*_{-i}) = \E[\totpulls{i}(n) - \toteffort{i}(n)] = \E[\totpulls{i}(n)] (1-(1-\meani)) \ge \meani  \E[\totpulls{i}(n)] \ge \meani 
\lpt n -o(n)   
\end{align}
\end{proof}

We now upper bound the utility of arm $i$ given given $S^*_{-i}$:
\begin{claim}
For any possible strategy profile $S_i$: 
\begin{align}
    u_i(S_i,S^*_{-i}) \leq \meani \lpt n + o(n)
\end{align}
\end{claim}
\begin{proof}
We begin with the following lemma: 
\begin{lemma}
Given $S^*_i$ and that the MAB algorithm satisfies linear pulls and relaxed monotonicity, then for any possibly strategy $S_i$, we have that $\E[\totpulls{i}(n)|S_i,S^*_{-i}]\leq \lpt n + o(n)$. 
\end{lemma}
By the linear pulls property we have $\E[\totpulls{i}(n)|S^*_i,S^*_{-i}] \leq \lpt n + o(n)$. Since the algorithm satisfies relaxed monotonicity, it follows that arm $i$ can maximize its number of pulls up to an $o(n)$ additive term by always giving a reward of $1$ whenever pulled and therefore for any possible strategy $S_i$, we have $\E[\totpulls{i}(n)|S_i,S^*_{-i}] \leq \E[\totpulls{i}(n)|S^*_i,S^*_{-i}] + o(n)\leq \lpt n + o(n)$
\end{proof}
For arm $i$ to have a utility $u_i=\Omega(n)$, then $\E[T_i(n)] \ge \alpha n$ where $\alpha$ is a constant. Since the other arms follow strategy $S^*_{-i}$, then we have a stochastic MAB instance with $\mu^*=1$, thus by the sharp robustness property it follows that if $\E[T_i(n)] \ge \alpha n$, then $C_i(n)>\alpha (1-\meani)n - o(n)$ and therefore $u_i(S_i,S^*_{-i})\leq \alpha \meani n + o(n)$. By the above lemma $\alpha$ has a maximum value of $\alpha=\lpt$ and therefore  $u_i(S_i,S^*_{-i})\leq  \meani \lpt n + o(n)$.   

Now we prove that linear pulls is necessary: 
\begin{theorem}
If a MAB algorithm $\alg$ does not satisfy linear pulls then $S^*$ cannot be a strong approximate equilibrium.   
\end{theorem}
\begin{proof}
Since the algorithm does not satisfy linear pulls, then if $S^*$ is followed then $\exists i \in [k]$ such that $\E[\totpulls{i}(n)]=o(n)$ which implies that $u_i \leq \E[\totpulls{i}(n)] = o(n)$ and therefore we do not have a strong approximate equilibrium under $S^*$.
\end{proof}

Now we prove that relaxed monotonicity is necessary: 
\begin{theorem}
If a MAB algorithm $\alg$ is not monotonic then $S^*$ cannot be an approximate equilibrium.   
\end{theorem}
\begin{proof}
For any arm $i$ that follows $S^*_i$ given $S^*_{-i}$, then $u_i(S^*_i,S^*_{-i}) \leq \meani \E[\totpulls{i}(n)|S^*_i,S^*_{-i}]$. But since the algorithm is not monotonic, then there exists an arm $i$ for which deviating to $S_i$ can lead to $\E[\totpulls{i}(n)|S_i,S^*_{-i}] \ge \E[\totpulls{i}(n)|S^*_i,S^*_{-i}] + \Omega(n)$. Since the maximum reward is $1$, then $\E[\toteffort{i}(n)|S_i,S^*_{-i}] \leq (1-\meani) \E[\totpulls{i}(n)|S_i,S^*_{-i}]$ and therefore $u_i(S_i,S^*_{-i}) \ge \meani \E[\totpulls{i}(n)|S_i,S^*_{-i}] \ge \meani \E[\totpulls{i}(n)|S^*_i,S^*_{-i}] + \Omega(n) \ge u_i(S^*_i,S^*_{-i}) + \Omega(n)$. Therefore, $S^*$ is not an equilibrium. 
\end{proof}
\end{proof}

\paragraph{Comment on the above result:} Interestingly, we see that it is not necessary for the algorithm to be fair among the top arms, but to pull them for a linear number of times. It follows also that if a sharply robust algorithm satisfies the FATA property, then $\lpt = \frac{1}{k}, \ \forall i \in [k]$.










==> Sufficient.tex <==
\section{Sufficient Conditions for Best Performance Equilibrium}\label{sec:sufficient_for_best_perf}
We assume here that we are in the \emph{competition with information} setting. I.e.. $\bk>1$ and every arm $i \in \armstop$ knows that $\bk>1$ and that it belongs in $\armstop$. We further assume that $\bk$ is a constant for simplicity. 

\subsection{Performance Incentivizing MAB Algorithm} 
We now give general properties for MAB algorithms and then show that they are sufficient to lead to a best performance equilibrium. Let us begin with the first property: 
% \begin{definition}\label{def:sr}
% \textbf{Sharp Robustness}: A MAB algorithm is sharply robust if for any given sub-optimal arm $i$, if $\E[T_i(n)] \ge \alpha n$ where $\alpha$ is a constant, then the total effort spent by arm $i$ is at least $\toteffort{i}(n) > \alpha \di n - o(n)$, for any possible strategy profile followed by the arms. 
% \end{definition}

We note the following interesting implication: 
\begin{theorem}\label{th:sr_always_sb_regret}
Any sharply robust MAB algorithm has sublinear regret for all possible strategy profiles.
\end{theorem}
\begin{proof}
For stochastic bandits the regret can be written as $R(n)= \sum_{i} \di \E[\totpulls{i}(n)]$. But since effort is enabled in our model, the regret is $R(n) = \sum_{i} \Big(\di \E[\totpulls{i}(n)] - \E[C_i(n)] \Big)$. Clearly, to have linear regret $R(n) = \Omega(n)$, then a sub-optimal arm $i$ has to be pulled for a linear number of times. Therefore, $\E[\totpulls{i}(n)] = \alpha n + o(n)$, but definition (\ref{def:sr}) states that this can only happen if $\toteffort{i}(n)\ge \alpha \di n -o(n)$. Accordingly, arm $i$'s contribution to the regret would be $\di \E[\totpulls{i}(n)] - \E[C_i(n)] \leq \di ( \alpha n + o(n) ) - ( \alpha \di n -o(n) ) = o(n)$. 
\end{proof}
\textbf{Remark:} Theorem (\ref{th:sr_always_sb_regret}) shows that sharp robustness is sufficient to satisfy objective (2) of being \textbf{robust}. I.e., using a sharply robust algorithm we will never have sublinear regret regardless of the strategy profile.   

Now we give the second property 
\begin{definition}\label{def:fata}
\textbf{Fairness Among the Top Arms (FATA)}: When there exists a subset of arms $\armsr$ such that whenever $i \in \armsr$ is pulled then a reward of $r^*=\max_{t\in [n]} r_t$ is given, then a MAB algorithm is fair among the top arms (FATA) if $\forall i,i' \in \armsr: |\E[\totpulls{i}(n)]-\E[\totpulls{i'}(n)]|\leq o(n)$. 
\end{definition}

%%%% Old versio of FATA
% \begin{definition}\label{def:fata}
% \textbf{Fairness Among the Top Arms (FATA)}: When there exists a subset of arms $\armstop$ such that whenever $i \in \armstop$ is pulled then a reward of $r^*=\max_{t\in [n]} r_t$ is given, then a MAB algorithm is fair among the top arms (FATA) if $\forall i,i' \in \armstop \text{ and } \forall t\in[n]: |\totpulls{i}(t)-\totpulls{i'}(t)|\leq 1$. 
% \end{definition}

Now we give the third property
\begin{definition}\label{def:monotonic}
\textbf{Monotonicity}: A MAB algorithm satisfies monotonicity if for any strategy profile $S=(S_1,\dots,S_k)$, if an arm $i$ was to deviate to the best performance strategy $S^*_i$, then $\forall j \neq i: \E[\totpulls{j}(n)|S^*_i,S_{-i}]\leq \E[\totpulls{j}(n)|S_i,S_{-i}]$.
\end{definition}
% \textbf{Monotonicity}: For any strategy $S_{-i}$ followed by the arms other then $i$,  if arm $i$ deviates from strategy $S_i$ to $S'_i$ such that for the $\ell^{\text{th}}$ pull of arm $i$ the reward of $S'_i$ is $r^{\ell}_i(S'_i) = r^{\ell}_i(S_i) + {r'}^{\ell}_i$ where $\Pr[{r'}^{\ell}_i \ge 0]=1$ (non-negative), then $\E[\totpulls{i}(n)|S_i,S_{-i}] \leq \E[\totpulls{i}(n)|S'_i,S_{-i}]$. \SEI{an even more restrictive property is sufficient}. 
% \end{definition}
Note that monotonicity implies the following: 
\begin{fact}
If a MAB algorithm is monotonic, then $\E[\totpulls{i}(n)|S^*_i,S_{-i}]\ge \E[\totpulls{i}(n)|S_i,S_{-i}]$.
\end{fact}
\begin{proof}
    \begin{align*}
        & n = \E[\totpulls{i}(n)|S_i,S_{-i}] + \sum_{j \neq i} \E[\totpulls{j}(n)|S_i,S_{-i}] = \E[\totpulls{i}(n)|S^*_i,S_{-i}] + \sum_{j \neq i} \E[\totpulls{j}(n)|S^*_i,S_{-i}] \\ 
        & \implies \E[\totpulls{i}(n)|S^*_i,S_{-i}] - \E[\totpulls{i}(n)|S_i,S_{-i}] =  \sum_{j \neq i} \Big( \E[\totpulls{j}(n)|S_i,S_{-i}] - \E[\totpulls{j}(n)|S^*_i,S_{-i}] \Big) \ge 0  
    \end{align*}
where the last inequality follows by the monotonicity property. 
\end{proof}
Monotonicity essentially states that if an arm $i$ was to deviate to $S^*_i$, then the other arms would not get more pulls whereas it might get more pulls. We call an algorithm that satisfies the above properties \emph{performance incentivizing}. As we will show such algorithms lead to an equilibrium where arms perform at the top performance.  
\begin{definition}
\textbf{Performance Incentivizing}: A MAB algorithm is performance incentivizing if it satisfies sharp robustness, FATA, and monotonicity. 
\end{definition}
\paragraph{\textbf{Algorithms that do not have good equilibrium:}} Before we prove that performance incentivizing algorithms lead to a good equilibrium. It is worthwhile to point out some algorithms which violate the above properties and clearly do not lead to a good equilibrium. Specifically, the explore first (or explore then commit) \cite{lattimore2020bandit,slivkins2019introduction} and successive elimination \cite{slivkins2019introduction} algorithms are clearly not sharply robust and would not lead to a good equilibrium. To see that, note that both algorithms have a limited phase (of $o(n)$ rounds) in the beginning after which they pick an arm and stick to it for the rest of the horizon. Therefore, if an arm gives the maximum reward value during this phase and then stops giving any effort afterwards it could be pulled for $n-o(n)$ rounds using only $o(n)$ total effort.  


\subsection{Performance Incentivizing MAB Algorithms Lead to a Best Performance Equilibrium}
Before we prove the best performance equilibrium, we start with the following lemma about sharply robust algorithms: 
\begin{fact}\label{fact:sr_sub_pulls}
Suppose a sub-optimal arm $i$ cannot improve its rewards, i.e. $C_i(n)=0$, then $\E[\totpulls{i}(n)]=o(n)$ regardless of the strategies followed by the other arms. 
\end{fact}
\begin{proof}
By definition of sharp robustness for $\E[\totpulls{i}(n)]=\alpha n = \Omega(n)$, then $C_i(n) > \alpha n -o(n)$. Since $C_i(n)=0$, then $\E[\totpulls{i}(n)]=o(n)$.
\end{proof}
% We can conclude the following from the above fact: 
% \begin{corollary}\label{th:sr_sb_ordinary_2}
% Every sharply robust MAB algorithm has sublinear regret in the (ordinary) stochastic MAB setting.  
% \end{corollary}
% \begin{proof}
% In the stochastic MAB setting, each arm $i \in [k]$ samples a reward from its distribution $\Dist_i$ without modification and therefore $C_i(n)=0, \forall i \in [k]$. By the above fact, it follows that all sub-optimal arms will be pulled for a sublinear number of times and therefore the regret is sublinear.  
% \end{proof}


\begin{theorem}
Given the competition with information setting, if a MAB algorithm is performance incentivizing, then there exists a strategy profile $S^*$ where $\forall i \in \armsup: S_i=S^*_i$ is an approximate equilibrium and $P(n)=\maxall n -o(n)$. 
\end{theorem}
\begin{proof}
We begin with the following claim which upper bounds the number of pulls for all arms $i \in \arms-\armsup$: 
\begin{claim}
Given strategy profile $\Sbesthet$, then for any strategy profile $\Sbestheto$ followed by arms $i' \in \arms-\armsup$, we have $\E[\totpulls{i'}(n)|\Sbesthet,\Sbestheto]=o(n)$. 
\end{claim}
\begin{proof}
Fix any arm $i' \in \arms-\armsup$ and suppose it follows strategy $\Sbestahet{i'}$ of always giving its maximum possible reward value of $M_{i'}$. Therefore, the MAB instance has been reduced to one where $\forall i \in \armsup$ rewards are sampled from a deterministic distribution which always gives $\maxall$ and for $i' \in \arms-\armsup$ the reward is sampled from another deterministic distribution which always gives $M_i$. Therefore, the reward gap for $i'$ becomes $\Delta_{i'}=\maxall-M_{i'}$. Since arm $i'$ cannot generate a higher reward than $M_{i'}$, it follows that in this reduction that $C_{i'}=0$ and therefore by Fact (\ref{fact:sr_sub_pulls}) regardless of the strategy profile $S''$ followed by the other arms $j' \in \arms-\armsup, j'\neq i'$, we have $\E[\totpulls{i'}(n)|\Sbestahet{i'},\Sbesthet,S'']=o(n)$. 

Since the algorithm is monotonic it follows that $i'$ can maximize its number of pulls by always the maximum possible reward, i.e. strategy $\Sbestahet{i'}$. It follows that $\forall i' \in \arms-\armsup$ we have $\E[\totpulls{i'}(n)|\Sbesthet,\Sbestheto]=o(n) \ , \forall \Sbestheto$.   
\end{proof}
Therefore, for arms $i' \in \arms-\armsup$ given that $\forall i \in \armstop: S_i=S^*_i$, then since the set actions belongs to a compact space, there exists an equilibrium for arms $i' \in \arms-\armsup$ (although it would have $u_{i'}=o(n), \forall i' \in \arms-\armsup$). Now we lower bound the utility of arms $i \in \armsup$:
\begin{lemma}
\begin{align}
    u_i(S^*_i,S^*_{-i}) \ge (1+\meani-\maxall) \frac{n}{\bk} - o(n) 
\end{align}
\end{lemma}
\begin{proof}
By the above claim, it follows that only arms in $i \in \armsup$ can have $\E[\totpulls{i}(n)]=\Omega(n)$. Since all arms in $\armsup$ always give a reward of $\maxall$, then it follows by the FATA property that $\frac{n}{\bk}-o(n) \leq \E[\totpulls{i}(n)] \leq \frac{n}{\bk}+o(n)$, therefore we have:
\begin{align}
        u_i(S^*_i,S^*_{-i}) \ge \E[\totpulls{i}(n)] - \E[\toteffort{i}(n)] = \E[\totpulls{i}(n)] (1-(M_i-\meani)) = (1+\meani-\maxall) \frac{n}{\bk} - o(n) 
\end{align}
\end{proof}
We now upper bound the utility of an arm $i$ given $S^*_{-i}$: 
\begin{lemma}
\begin{align}
        u_i(S_i,S^*_{-i}) \leq (1+\meani-M_i) \frac{n}{\bk} + o(n)
\end{align}
\end{lemma}
\begin{proof}
We begin with the following lemma: 
\begin{lemma}
Given $S^*_i$ and that the MAB algorithm is FATA and Monotonic, then for any possible strategy $S_i$, we have that $\E[\totpulls{i}(n)]\leq \frac{n}{\bk}+o(n)$. 
\end{lemma}
Since the algorithm is monotonic, it follows that arm $i$ can maximize its number of pulls by always giving a reward of $\maxall$ whenever pulled. Further, since it is FATA and the other arms follow $S^*_i$, then $\E[\totpulls{i}(n)]\leq \frac{n}{\bk}+o(n)$. 
\end{proof}
For arm $i$ to have a utility $u_i=\Omega(n)$, then $\E[T_i(n)] \ge \alpha n$ where $\alpha$ is a constant. Since the other arms in $\armsup$ follow strategy $S^*_{-i}$, then we have a MAB instance with $\mu^*=\maxall$ and $\di=\maxall-\meani$, thus by the sharp robustness property it follows that if $\E[T_i(n)] \ge \alpha n$, then $C_i(n)>\alpha (\maxall-\meani)n - o(n)$ and therefore $u_i(S_i,S^*_{-i})\leq \alpha (1+\meani-\maxall) n + o(n)$. By the above lemma $\alpha$ has a maximum value of $\alpha=\frac{1}{\bk}$ and therefore  $u_i(S_i,S^*_{-i})\leq  (1+\meani-\maxall) \frac{n}{\bk} + o(n)$.    
\end{proof}
% % Now we prove the following theorem: 
% % \begin{theorem}\label{th:pi_hetro}
% % In the homogeneous setting, if a MAB algorithm is performance incentivizing, then strategy profile $S^*$ is an $o(n)$-equilibrium. 
% % \end{theorem}
% % \begin{proof}
% % We begin by lower bounding the utility of arm $i$ when it follows strategy $S^*_i$ given $S^*_{-i}$:

% % \begin{lemma}
% % \begin{align}
% %     u_i(S^*_i,S^*_{-i}) \ge \meani \frac{n}{k} - o(n) 
% % \end{align}
% % \end{lemma}

% % \begin{proof}
% % Since the algorithm satisfies the FATA property it follows that $\forall i,i' \in [k]: |\E[\totpulls{i}(n)]-\E[\totpulls{i'}(n)]|\leq o(n)$ and since the strategy profile is $S^*$ it follows that $\frac{n}{k}-o(n) \leq \E[\totpulls{i}(n)] \leq \frac{n}{k}+o(n)$, therefore we have: 
% % \begin{align}
% %     u_i(S^*_i,S^*_{-i}) = \E[\totpulls{i}(n) - \toteffort{i}(n)] = \E[\totpulls{i}(n)] (1-(1-\meani)) \ge \meani ( \frac{n}{k}- o(n)) \ge \meani \frac{n}{k} - o(n) 
% % \end{align}
% % \end{proof}

% % We now upper bound the utility of arm $i$ given given $S^*_{-i}$:
% % \begin{lemma}
% % For any possible strategy profile $S_i$: 
% % \begin{align}
% %     u_i(S_i,S^*_{-i}) \leq \meani \frac{n}{k} + o(n)
% % \end{align}
% % \end{lemma}
% % \begin{proof}
% % We begin with the following lemma: 
% % \begin{lemma}
% % Given $S^*_i$ and that the MAB algorithm is FATA and Monotonic, then for any possible strategy $S_i$, we have that $\E[\totpulls{i}(n)]\leq \frac{n}{k}+o(n)$. 
% % \end{lemma}
% % Since the algorithm is monotonic, it follows that arm $i$ can maximize its number of pulls by always giving a reward of $1$ whenever pulled. Further, since it is FATA and the other arms follow $S^*_i$, then $\E[\totpulls{i}(n)]\leq \frac{n}{k}+o(n)$. 
% % \end{proof}
% For arm $i$ to have a utility $u_i=\Omega(n)$, then $\E[T_i(n)] \ge \alpha n$ where $\alpha$ is a constant. Since the other arms follow strategy $S^*_{-i}$, then we have a stochastic MAB instance\footnote{By stochastic MAB instance we mean that each arm other than $i$ when pulled will give a reward from an iid distribution} with $\mu^*=1$, thus by the sharp robustness property it follows that if $\E[T_i(n)] \ge \alpha n$, then $C_i(n)>\alpha (1-\meani)n - o(n)$ and therefore $u_i(S_i,S^*_{-i})\leq \alpha \meani n + o(n)$. By the above lemma $\alpha$ has a maximum value of $\alpha=\frac{1}{k}$ and therefore  $u_i(S_i,S^*_{-i})\leq  \meani \frac{n}{k} + o(n)$.    
% \end{proof}

 

\input{UCB1_properties}









% \subsection{Sufficient Conditions for Best Performance Equilibrium (Heterogeneous $\bk>1$ with information)}
% Before we prove the equilibrium for this setting, we start with the following lemma about sharply robust algorithms: 
% \begin{fact}\label{fact:sr_sub_pulls}
% Suppose a sub-optimal arm $i$ cannot improve its rewards, i.e. $C_i(n)=0$, then $\E[\totpulls{i}(n)]=o(n)$ regardless of the strategies followed by the other arms. 
% \end{fact}
% \begin{proof}
% By definition of sharp robustness for $\E[\totpulls{i}(n)]=\alpha n = \Omega(n)$, then $C_i(n) > \alpha n -o(n)$. Since $C_i(n)=0$, then $\E[\totpulls{i}(n)]=o(n)$.
% \end{proof}
% We can conclude the following from the above fact: 
% \begin{corollary}\label{th:sr_sb_ordinary_2}
% Every sharply robust MAB algorithm has sublinear regret in the (ordinary) stochastic MAB setting.  
% \end{corollary}
% \begin{proof}
% In the stochastic MAB setting, each arm $i \in [k]$ samples a reward from its distribution $\Dist_i$ without modification and therefore $C_i(n)=0, \forall i \in [k]$. By the above fact, it follows that all sub-optimal arms will be pulled for a sublinear number of times and therefore the regret is sublinear.  
% \end{proof}


% \begin{theorem}
% In the heterogeneous setting with information, if a MAB algorithm $\alg$ satisfies sharp robustness, FATA, and monotonicity, then there exists a strategy profile $S^*_M$ where $\forall i \in \armsup: S_i=S^*_i$ is an $o(n)$-equilibrium and $P(n)=\maxall n -o(n)$. 
% \end{theorem}
% \begin{proof}
% \SEI{add there exists an equilibrium for the non-top arms}
% We begin by the following claim which upper bounds the number of pulls for all arms $i \in \arms-\armsup$: 
% \begin{claim}
% Given strategy profile $\Sbesthet$, then for any strategy profile for $\Sbestheto$ followed by arms $i' \in \arms-\armsup$, we have $\E[\totpulls{i'}(n)|\Sbesthet,\Sbestheto]=o(n)$. 
% \end{claim}
% \begin{proof}
% Fix any arm $i' \in \arms-\armsup$ and suppose it follows strategy $\Sbestahet{i'}$ of always giving its maximum possible reward value of $M_{i'}$. Therefore, the MAB instance has been reduced to one where $\forall i \in \armsup$ rewards are sampled from a deterministic distribution which always gives $\maxall$ and for $i' \in \arms-\armsup$ the reward is sampled from another deterministic distribution which always gives $M_i$. Therefore, the reward gap for $i'$ becomes $\Delta_{i'}=\maxall-M_{i'}$. Since arm $i'$ cannot generate a higher reward than $M_{i'}$, it follows that in this reduction that $C_{i'}=0$ and therefore by Fact (\ref{fact:sr_sub_pulls}) regardless of the strategy profile $S''$ followed by the other arms $j' \in \arms-\armsup, j'\neq i'$, we have $\E[\totpulls{i'}(n)|\Sbestahet{i'},\Sbesthet,S'']=o(n)$. 

% Since the algorithm is monotonic it follows that $i'$ can maximize its rewards by always the maximum possible reward, i.e. strategy $\Sbestahet{i'}$. Therefore, $\forall i' \in \arms-\armsup$ we have $\E[\totpulls{i'}(n)|\Sbesthet,\Sbestheto]=o(n) \ , \forall \Sbestheto$.   
% \end{proof}
% Now we lower bound the utility of arms $i \in \armsup$:
% \begin{lemma}
% \begin{align}
%     u_i(S^*_i,S^*_{-i}) \ge (1+\meani-\maxall) \frac{n}{\bk} - o(n) 
% \end{align}
% \end{lemma}
% \begin{proof}
% By the above claim it follows that only arms in $i \in \armsup$ can have $\E[\totpulls{i}(n)]=\Omega(n)$. Since all arms in $\armsup$ always give a reward of $\maxall$, then it follows by the FATA property that $\frac{n}{\bk}-o(n) \leq \E[\totpulls{i}(n)] \leq \frac{n}{\bk}+o(n)$, therefore we have:
% \begin{align}
%         u_i(S^*_i,S^*_{-i}) \ge \E[\totpulls{i}(n)] - \E[\toteffort{i}(n)] = \E[\totpulls{i}(n)] (1-(M_i-\meani)) = (1+\meani-\maxall) \frac{n}{\bk} - o(n) 
% \end{align}
% \end{proof}
% We now upper bound the utility of an arm $i$ given $S^*_{-i}$: 
% \begin{lemma}
% \begin{align}
%         u_i(S_i,S^*_{-i}) \leq (1+\meani-M_i) \frac{n}{\bk} + o(n)
% \end{align}
% \end{lemma}
% \begin{proof}
% We begin with the following lemma: 
% \begin{lemma}
% Given $S^*_i$ and that the MAB algorithm is FATA and Monotonic, then for any possibly strategy $S_i$, we have that $\E[\totpulls{i}(n)]\leq \frac{n}{\bk}+o(n)$. 
% \end{lemma}
% Since the algorithm is monotonic, it follows that arm $i$ can maximize its number of pulls by always giving a reward of $\maxall$ whenever pulled. Further, since it is FATA and the other arms follow $S^*_i$, then $\E[\totpulls{i}(n)]\leq \frac{n}{\bk}+o(n)$. 
% \end{proof}
% For arm $i$ to have a utility $u_i=\Omega(n)$, then $\E[T_i(n)] \ge \alpha n$ where $\alpha$ is a constant. Since the other arms in $\armsup$ follow strategy $S^*_{-i}$, then we have a MAB instance with $\mu^*=\maxall$ and $\di=\maxall-\meani$, thus by the sharp robustness property it follows that if $\E[T_i(n)] \ge \alpha n$, then $C_i(n)>\alpha (\maxall-\meani)n - o(n)$ and therefore $u_i(S_i,S^*_{-i})\leq \alpha (1+\meani-\maxall) n + o(n)$. By the above lemma $\alpha$ has a maximum value of $\alpha=\frac{1}{\bk}$ and therefore  $u_i(S_i,S^*_{-i})\leq  (1+\meani-\maxall) \frac{n}{\bk} + o(n)$.    
% \end{proof}

==> conclusion.tex <==
\section{Conclusion}
We studied a strategic version of the multi-armed bandit problem which captures various applications such as online labor markets.
We showed that if a MAB algorithm is performance incentivizing then it induces an asymptotic equilibrium where the arms give their top performance while at the same time being robust, i.e., having a guarantee on the minimum revenue obtained even for non-equilibrium strategy profiles provided we have at least one honest agent. Furthermore, under a reasonable condition we showed that there does not exists an equilibrium that leads to the principle obtaining sub-optimal revenue. Finally, to cope with the setting where the top performance level is unknown, we introduced an algorithm that combines elements from second price auctions with performance incentivizing algorithms. 

% Finally, we considered more general cost functions and showed how some of our results still hold in that setting. Exploring cost functions in more depth, using contract-theoretic ideas and introducing dynamic consideration such as time varying agent characteristics in the model are interesting directions for future work.

==> cost_func_design.tex <==
\section{Cost Function Design}
\SE{Does not Work}
Let $g_i(m_i)=\E[c_i(m_i-r_i)]$, then by definition we have $g_i(M_i^{(c)})=0$. We make the following assumption on $g_i$:
\begin{assumption}
$g_i$ is $\rho_i$-Lipshitz, i.e. $\forall m,m': |g_i(m)-g_i(m')|\leq \rho_i|m-m'|$.
\end{assumption}
As before $c$ is also increasing. 

We assume the principle knows the upper bound on the Lipshitz constants for all arms and that this Lipshitz constant is independent on the horizon $\Theta(1)$. Denote this upper bound by $\rho \ge \max_{i\in [k]} \rho_i$. 

We want to maximize the following function to incentivize giving $\mic$: 
\begin{align*}
    Q(m_i) = f(m_i) (\rho + 1-g_i(m_i))
\end{align*}
Note that $f(m_i)$ plays the role of $m^\alpha_i$, we should also reward with $\rho$ rounds instead of 2. We chose $f(m_i)=m_i \ln(n)$. This means an increase by an order for $\ln(n)$ for the pulls. Accordingly, the function is: 
\begin{align*}
    Q(m_i) = m_i \ln(n) (\rho + 1-g_i(m_i))
\end{align*}
Now we show the following facts: 
\begin{fact}
$Q(\mic) = \mic \ln(n) \rho
\end{fact}
\begin{proof}
By definition of $\mic$, we would have $1-g_i(\mic)=0$ and the expression follows. 
\end{proof}
\begin{fact}
$\forall m_i>\mic: Q(m_i) < Q(\mic)$.
\end{fact}
\begin{proof}
By definition of $\mic$ and that fact that $g_i$ is increasing, then we would have $1-g_i(m_i)\leq 1-g_i(\mic)=0$ and therefeore expression follows. 
\end{proof}





==> eps_greedy_properties.tex <==
\section{$\epsilon$-Greedy is Performance Incentivizing}\label{sec:eps_greedy_PI}

% \begin{algorithm}
% Play each arm once for the first $k$ rounds.\\
% In a given round $t>k$:  \\
% \ \ (1) Sample a Bernoulli random variable $s_t$ from $Bern(\epsilon)$. \\
% \ \ (2) If $s_t=1$, then a pick an arm uniformly at random. \\
% \ \ (3) If $s_t=0$, then sample an arm uniformly at random from the set of arms with maximum empirical mean. 
% \caption{\textsc{$\epsilon$-Greedy}}\label{alg:eps_greedy}
% \end{algorithm}

\SE{removed algorithm block}

Note that $\epsilon=c (k \ln(n))^{\frac{1}{3}} n^{\frac{-1}{3}}$ where $c=32$ is a constant. Further, throughout the derivations for an arm $i$ we denote by $T^R_i(t)$ and $T^E_i(t)$ the number of pulls up to and including round $t$ that arm $i$ receives in exploration rounds (when $s_t=1$) and in exploitation rounds (when $s_t=0$), respectively. 
%\sscomment{perhaps might be better to define more in a generic manner: $T_i^R(t)$ for any $t \in [n]$? (as is used below)}

We start by proving the regret bound for $\epsilon$-greedy. Note that this bound is for the ordinary setting of stochastic bandits without the effort modification. In the analysis we use asymptotic notation to avoid specifying the constants which would be more cumbersome.   
% \begin{theorem}\label{th:eps_greedy_regretbound}
% $\epsilon$-greedy has a regret of $O(n^{\frac{2}{3}} k^{\frac{1}{3}} (\ln(n))^{\frac{1}{3}})$.
% \end{theorem}
% \begin{proof}
% We start by defining the $\ce$. Under the $\ce$ we have:
% \begin{align}
% \forall i \in \arms, \forall t \in [n]: \ \ & |\meanit{t}-\mu_i| \leq \sqrt{\frac{2\ln(n)}{T_i(t)}} \label{eq:ce_eps_1} \\ 
% \forall i \in \arms, \forall t \ge  n^{\frac{2}{3}} k^{\frac{1}{3}} (\ln(n))^{\frac{1}{3}}: \ \ & T^R_i(t) \ge  \frac{c}{2} k^{-\frac{2}{3}} (\ln(n))^{\frac{1}{3}} n^{\frac{-1}{3}} t  \label{eq:ce_eps_2}
% \end{align}
% \end{proof}
% We want to show that the clean event happens with high probability. We start by proving the second inequality \eqref{eq:ce_eps_2}: 
% \begin{claim}\label{cl:eps_second}
% \begin{align}
%      \Pr\Big(\E[T^R_i(t)] - T^R_i(t) \ge \frac{1}{2} c k^{-\frac{2}{3}} (\ln(n))^{\frac{1}{3}} n^{\frac{-1}{3}} t \Big) \leq \frac{1}{n^4}
% \end{align}
% \end{claim}
% \begin{proof}
% We start by finding the $\E[T^R_i(t)]$: 
% \begin{align*}
%     \E[T^R_i(t)] & = \sum_{s=1}^t \frac{c k^{\frac{1}{3}} (\ln(n))^{\frac{1}{3}} n^{\frac{-1}{3}}}{k} \\ 
%                  & = c k^{\frac{-2}{3}} (\ln(n))^{\frac{1}{3}} n^{\frac{-1}{3}} t 
% \end{align*}
% Now we apply a tail inequality of Theorem \ref{th:cherbound}:
% \begin{align*}
%     \Pr\Big(T^R_i(t) \leq \frac{1}{2}  \E[T^R_i(t)]\Big) & \leq \exp{(-\frac{1}{8} \E[T^R_i(t)])} \\ 
%     & = \exp{(-\frac{1}{8} c k^{\frac{-2}{3}} (\ln(n))^{\frac{1}{3}} n^{\frac{-1}{3}} t)} \\ 
%     & \leq \exp(-4 \ln(n)) && \text{(since $t \ge n^{\frac{2}{3}} k^{\frac{1}{3}} (\ln(n))^{\frac{1}{3}}$)}  \\
%     & = \frac{1}{n^4}
% \end{align*}
% Now we can prove that the $\ce$ happens with high probability: 
% \begin{claim}\label{cl:cleanevent_greedy}
% \begin{align*}
%     \Pr(\ce) \ge 1-\frac{3}{n^2}
% \end{align*}
% \end{claim}
% \begin{proof}
% Note that for the first condition in the clean event \eqref{eq:ce_eps_1} we can show that it fails for a given arm and round with probability at most $\frac{2}{n^4}$ using the same proof of Claim \ref{cl:ucb_clean_event} for UCB. Now consider some arm $i \in \arms$ and round $t  \ge n^{\frac{2}{3}} k^{\frac{1}{3}} (\ln(n))^{\frac{1}{3}}$, then by Claim \ref{cl:eps_second} we have the probability that inequality \eqref{eq:ce_eps_2} is upper bounded by $\frac{1}{n^4}$. Therefore, we can bound the $\be$ event (which is the complement of the $\ce$) using the union bound as follows:
% \begin{align*}
%     \Pr(\be) \leq \frac{3}{n^4} k n \leq \frac{3}{n^2}
% \end{align*}
% Therefore, we have $\Pr(\ce)\ge 1-\frac{3}{n^2}$. 
% \end{proof}

% Now under the clean event we can upper bound the regret as follows:
% \begin{align}
%     1 + \sum_{t=1}^n \E[\Delta_{I_{t+1}}] & \leq 1 + \sum_{t=1}^{\ceil{n^{\frac{2}{3}} k^{\frac{1}{3}} (\ln(n))^{\frac{1}{3}}}} (1) + \sum_{t=\ceil{n^{\frac{2}{3}} k^{\frac{1}{3}} (\ln(n))^{\frac{1}{3}}} + 1}^{n} \E[\Delta_{I_{t+1}}] \\ 
%     & \leq 2 + n^{\frac{2}{3}} k^{\frac{1}{3}} (\ln(n))^{\frac{1}{3}} + \sum_{t=\ceil{n^{\frac{2}{3}} k^{\frac{1}{3}} (\ln(n))^{\frac{1}{3}}} + 1}^{n} \Big( \epsilon (1)+ (1-\epsilon) \sum_{i \in \arms} \Delta_i \Pr(I_{t+1}=i) \Big) \\ 
%     & \leq 2 + n^{\frac{2}{3}} k^{\frac{1}{3}} (\ln(n))^{\frac{1}{3}} + \epsilon n + \sum_{t=\ceil{n^{\frac{2}{3}} k^{\frac{1}{3}} (\ln(n))^{\frac{1}{3}}} + 1}^{n} \Big( \sum_{i \in \arms} \Delta_i \Pr(I_{t+1}=i) \Big) \\ 
%     & \leq 2 + n^{\frac{2}{3}} k^{\frac{1}{3}} (\ln(n))^{\frac{1}{3}} + c n^{\frac{2}{3}} (k \ln(n))^{\frac{1}{3}} + \sum_{t=\ceil{n^{\frac{2}{3}} k^{\frac{1}{3}} (\ln(n))^{\frac{1}{3}}} + 1}^{n} \Big( \sum_{i \in \arms} \Delta_i \Pr(I_{t+1}=i) \Big) \label{eq:eps_reg_bound_inter_1} 
% \end{align}
% Now suppose that a sub-optimal arm $i$ is pulled for a round $t\ge \ceil{n^{\frac{2}{3}} k^{\frac{1}{3}} (\ln(n))^{\frac{1}{3}}}$, then  by the clean event we must have: 
% \begin{align*}
%     \meanit{t} & \ge \hat{\mu}_{i^*}(t) \\ 
%     \meanit{t} & \leq \mu_i + \sqrt{\frac{2 \ln(n)}{\totpulls{i}(t)}} \\
%     \hat{\mu}_{i^*}(t) & \ge \mu_{i^*} - \sqrt{\frac{2 \ln(n)}{\totpulls{i^*}(t)}}
% \end{align*}
% Therefore, we must have:
% \begin{align}
%     \Delta_i = \mu_{i^*} - \mu_i & \leq \sqrt{\frac{2 \ln(n)}{\totpulls{i^*}(t)}} + \sqrt{\frac{2 \ln(n)}{\totpulls{i}(t)}} \\ 
%     & \leq 4 \sqrt{\frac{(\ln(n))^{\frac{2}{3}}}{c k^{\frac{-2}{3}} n^{\frac{-1}{3}} t}} && \tag{from inequality \eqref{eq:ce_eps_2}} \\ 
%     & \leq \frac{4}{\sqrt{c}} k^{\frac{1}{3}} (\ln(n))^{\frac{1}{3}} n^{\frac{1}{6}} t^{\frac{-1}{2}} 
% \end{align}
% Therefore, the bound in \eqref{eq:eps_reg_bound_inter_1} becomes:
% \begin{align*}
%     2 + n^{\frac{2}{3}} k^{\frac{1}{3}} (\ln(n))^{\frac{1}{3}} + c n^{\frac{2}{3}} (k \ln(n))^{\frac{1}{3}} + \sum_{t=\ceil{\frac{8^3}{c^6} \ln(n)} + 1}^{n} \frac{4}{\sqrt{c}} k^{\frac{1}{3}} (\ln(n))^{\frac{1}{3}} n^{\frac{1}{6}} t^{\frac{-1}{2}}
% \end{align*}
% Since $\sum_{t=1}^n t^{\frac{-1}{2}} \leq 1 + \int_{1}^{n}  t^{\frac{-1}{2}} dt \leq 2 n^{\frac{1}{2}}$, then the bound under the clean event becomes: 
% \begin{align*}
%     & 2 + n^{\frac{2}{3}} k^{\frac{1}{3}} (\ln(n))^{\frac{1}{3}} + c n^{\frac{2}{3}} (k \ln(n))^{\frac{1}{3}} + \frac{8}{\sqrt{c}} n^{\frac{2}{3}} k^{\frac{1}{3}} (\ln(n))^{\frac{1}{3}}  \\ 
%     & = O(n^{\frac{2}{3}} k^{\frac{1}{3}} (\ln(n))^{\frac{1}{3}})
% \end{align*}
% Therefore the final regret upper bound is: 
% \begin{align*}
%     R(n) & \leq \Pr(\ce) \cdot O(n^{\frac{2}{3}} k^{\frac{1}{3}} (\ln(n))^{\frac{1}{3}})  + (1-\Pr(\ce)) 
%     \cdot n \\ 
%     & \leq (1) \cdot O(n^{\frac{2}{3}} k^{\frac{1}{3}} (\ln(n))^{\frac{1}{3}}) + \frac{3}{n^2} \cdot n \\
%     & = O(n^{\frac{2}{3}} k^{\frac{1}{3}} (\ln(n))^{\frac{1}{3}})
% \end{align*}
% \end{proof}

% Now we prove that $\epsilon$-greedy is sharply adaptive: 
% \begin{theorem}\label{th:eps_greedy_sr}
% $\epsilon$-Greedy is sharply adaptive. 
% \end{theorem}






==> macros.tex <==
%%% \SE{your comment}, \AS{your comment}
\newcommand{\SE}[1]{{\color{blue} (\textbf{SE:} #1)}}
\newcommand{\SEI}[1]{{\color{red} (\textbf{SEI Comment:} #1)}}
\newcommand{\SH}[1]{{\color{teal} (\textbf{SH Comment:} #1)}}
\newcommand{\AS}[1]{{\color{red} (\textbf{AS Comment:} #1)}}
\newcommand{\eps}{\varepsilon}
\newcommand{\todo}[1]{\textcolor{red}{TODO: #1}}

\newcommand{\feas}{\textsc{FeasBid}}
\newcommand{\rev}{\textsc{RevMaxBid}}
\newcommand{\parans}[1]{{\left(#1 \right)}}
\newcommand{\paranm}[1]{{\left\{#1 \right\}}}
\newcommand{\paranl}[1]{{\left[#1 \right]}}
\newcommand{\Ex}[1]{{\mathbb{E} \left[ #1 \right]}}
\newcommand{\Exu}[2]{\ensuremath{\mathbb{E}_{#1}\left[#2\right]}}
\newcommand{\rtilde}{\Tilde{r}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}


\DeclareMathOperator{\indic}{\mathds{1}}




\DeclareMathOperator{\E}{\mathbb{E}}
\DeclareMathOperator{\Prob}{\mathbb{P}}

\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}

% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{assumption}{Assumption}[section]
% \newtheorem{condition}{Condition}[section]
% \newtheorem{claim}{Claim}[section]
% \newtheorem{fact}{Fact}[section]
% \newtheorem{observ}{Observation}[section]
% \newtheorem{definition}{Definition}[section]
% \newtheorem{OP}{Theorem}[section]
% \newtheorem{lemma}{Lemma}[section]
% \newtheorem{corollary}{Corollary}[section]
% \newtheorem{note}{Note}

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{construction}[theorem]{Construction}
\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{algorithm}[theorem]{Algorithm}
\newtheorem{reduction}[theorem]{Reduction}
\newtheorem{invariant}[theorem]{Invariant}
\newtheorem{extension}[theorem]{Extension}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{condition}[theorem]{Condition}

\newtheorem*{theorem*}{Theorem}
\newtheorem*{lemma*}{Lemma}
\newtheorem{claim*}{Claim}

\theoremstyle{definition}
\newtheorem*{definition*}{Definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{example}[theorem]{Example}

\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{discussion}[theorem]{Discussion}
\newtheorem*{remark*}{Remark}
\newtheorem*{property*}{Property}
\newtheorem{exercise}{Exercise}[section]
\newtheorem*{problem*}{Problem formulation}

% Custom Theorem used in Restatement
\newtheorem{innercustomthm}{Restatement of Theorem}
\newenvironment{customthm}[1]
  {\renewcommand\theinnercustomthm{#1}\innercustomthm}
  {\endinnercustomthm}

\usepackage{stackengine}
\newcommand\barbelow[1]{\stackunder[1.2pt]{$#1$}{\rule{.8ex}{.075ex}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MAB Macros: 
\DeclareMathOperator{\bk}{\mathnormal{k_{\text{top}}}}     %\DeclareMathOperator{\bk}{\mathnormal{\bar{k}}}
\DeclareMathOperator{\di}{\mathnormal{\Delta_i}}
\DeclareMathOperator{\gap}{\mathnormal{\Delta}}
\DeclareMathOperator{\gapsi}{\mathnormal{\Delta_i^*}}
\newcommand{\empi}[1]{\mathnormal{\hat{\mu}_i({#1})}}
\newcommand{\emp}[1]{\mathnormal{\hat{\mu}_{#1}}}
\newcommand{\modif}[1]{\mathnormal{\widetilde{\mu}_{#1}}}
\DeclareMathOperator{\armt}{\mathnormal{I}_t}
\DeclareMathOperator{\arm}{\mathnormal{A}}
\DeclareMathOperator{\arms}{\mathcal{A}}
\DeclareMathOperator{\armsub}{\mathcal{A}_{sub-opt}}
\DeclareMathOperator{\pullt}{\mathnormal{I_t}}
%\DeclareMathOperator{\totit}{\mathnormal{T_i(t)}}


\DeclareMathOperator{\Dist}{\mathcal{D}}
\DeclareMathOperator{\alg}{\mathcal{A}}


\DeclareMathOperator{\meani}{\mathnormal{\mu_i}}
\newcommand{\totit}[1]{\mathnormal{T_i(#1)}}
\newcommand{\totpulls}[1]{\mathnormal{T_{#1}}}
\newcommand{\toteffort}[1]{\mathnormal{C_{#1}}}
\newcommand{\hmeani}{\mathnormal{\hat{\mu}_i}}
\newcommand{\meanit}[1]{\mathnormal{\hat{\mu}_i(#1)}}
%\newcommand{\meanit}[1]{\mathnormal{\hat{\mu}_i}}
\newcommand{\fmeanit}[1]{\mathnormal{\widetilde{\mu}_i(#1)}}
\newcommand{\ucbit}[2]{\mathnormal{UCB_{#1}(\mathnormal{#2})}}
\newcommand{\ucbi}[1]{\mathnormal{UCB_{#1}}}
\newcommand{\mech}{\mathcal{M}}

\newcommand{\estmean}[1]{\mathnormal{\hat{\mu}_{#1}}}



\DeclareMathOperator{\armsup}{\mathcal{A}_{\text{top}}}
\DeclareMathOperator{\armsdown}{\barbelow{\mathcal{A}}}

\DeclareMathOperator{\armstop}{\mathcal{A}_{\text{top}}}

\DeclareMathOperator{\armsr}{\mathcal{A}_\mathnormal{r^*}}


\DeclareMathOperator{\bci}{\mathnormal{\bar{C}_i}}
\DeclareMathOperator{\probeps}{\mathnormal{p(\epsilon,S_i)}}


\DeclareMathOperator{\maxi}{\mathnormal{M_i}}
\DeclareMathOperator{\maxall}{\mathnormal{M_{\text{top}}}}  %\DeclareMathOperator{\maxall}{\mathnormal{\bar{M}}}

\DeclareMathOperator{\armsmaxm}{\mathnormal{\mathcal{A}_{\bar{M}}}}
\DeclareMathOperator{\ks}{\mathnormal{\bar{k}}}

\DeclareMathOperator{\kbar}{\mathnormal{k_{\text{top}}}}     %\DeclareMathOperator{\kbar}{\mathnormal{\bar{k}}}


\DeclareMathOperator{\spucb}{\mathnormal{S^{\text{SP+PI}}}}



\DeclareMathOperator{\pullseq}{\mathcal{P}}


\newcommand{\norm}[1]{\left\lVert#1\right\rVert}



\DeclareMathOperator{\Vaug}{\mathnormal{V^{\text{aug}}}}
\DeclareMathOperator{\Aaug}{\mathnormal{A^{\text{aug}}}}

%%%%%
\DeclareMathOperator{\wv}{\mathnormal{w(v)}}
\DeclareMathOperator{\weights}{\mathnormal{W}}
\DeclareMathOperator{\dw}{\mathnormal{d_{\weights}}}
\newcommand{\wvs}[1]{w(#1)}
\DeclareMathOperator{\pop}{\boldsymbol{W}}



\DeclareMathOperator{\ac}{\mathnormal{A_c}}
\DeclareMathOperator{\acest}{\mathnormal{\hat{A}_c}}
\DeclareMathOperator{\unit}{\mathnormal{\boldsymbol{u}}}




\DeclareMathOperator{\qa}{\mathnormal{q_{\alpha}}}

\DeclareMathOperator{\lpt}{\mathnormal{\theta^{\alg}_i}}



% \DeclareMathOperator{\Sopt}{\mathnormal{\widetilde{S}}}
% \DeclareMathOperator{\Sopta}{\mathnormal{\widetilde{S}^*}}
% \DeclareMathOperator{\Soptb}{\mathnormal{\widetilde{S}^{\prime}}}


\newcommand{\Sbest}{\mathnormal{S^*}}
\newcommand{\Sbesthet}{\mathnormal{S^*}} % {\mathnormal{\bar{S}^*_M}}
\newcommand{\Sbestheti}[1]{\mathnormal{S^*_{#1}}} 
\newcommand{\Sbestheticost}[1]{\mathnormal{S^{*}_{#1}}} 



\newcommand{\Sbestheto}{\mathnormal{{S'}}}


\newcommand{\Sbesta}[1]{\mathnormal{S^*_{#1}}}
\newcommand{\Sbestahet}[1]{\mathnormal{S^{*}_{#1}}}

\DeclareMathOperator{\ce}{\term{Clean \ Event}}
\DeclareMathOperator{\be}{\term{Bad \ Event}}


\DeclareMathOperator{\tcal}{\mathcal{T}}



\DeclareMathOperator{\armssl}{\mathnormal{\mathcal{A}_{o(n)}}}
\DeclareMathOperator{\armstcal}{\mathnormal{\mathcal{A}^{\tcal}_{\Omega(n)}}}
\DeclareMathOperator{\armsntcal}{\mathnormal{\mathcal{A}_{\Omega(n)}}}



\newcommand{\mic}{\mathnormal{M_i^{f}}}
\newcommand{\mjc}{\mathnormal{M_j^{f}}}
\newcommand{\kic}{\mathnormal{k_{top}}}
\DeclareMathOperator{\armstopc}{\mathnormal{\mathcal{A}_{\text{top}}}}
\DeclareMathOperator{\maxallc}{\mathnormal{M_{\text{top}}}}  %\DeclareMathOperator{\maxall}{\mathnormal{\bar{M}}}

\newcommand{\mlow}{\mathnormal{m_{\text{min}}}}


\newcommand{\pc}[1]{\mathnormal{\text{PullCount}_{#1}}} 
\newcommand{\rpi}[1]{\mathnormal{\tilde{r}_p({#1})}}
\newcommand{\tildr}{\mathnormal{\tilde{r}}}





\DeclareMathOperator{\topt}{\mathcal{T}^{\text{OPT}}}
\DeclareMathOperator{\tsubopt}{\mathcal{T}^{\text{sub}}}

\newcommand{\toptj}[1]{\mathcal{T}^{\text{OPT}}_{#1}}
\newcommand{\tsuboptj}[1]{\mathcal{T}^{\text{sub}}_{#1}}


\DeclareMathOperator{\popt}{\mathcal{P}^{\text{OPT}}}
\DeclareMathOperator{\psubopt}{\mathcal{P}^{\text{sub}}}
\newcommand{\poptj}[1]{\mathcal{P}^{\text{OPT}}_{#1}}
\newcommand{\psuboptj}[1]{\mathcal{P}^{\text{sub}}_{#1}}


\newcommand{\thetaopti}[1]{\mathnormal{\theta^{\text{OPT}}_{#1}}}
\newcommand{\thetasubopti}[1]{\mathnormal{\theta^{\text{sub-OPT}}_{#1}}}
\newcommand{\avgi}[1]{\mathnormal{\text{avg}^{\text{sub-OPT}}_{#1}}}


\DeclareMathOperator{\honestarm}{\mathnormal{h}_{\text{max}}}
\DeclareMathOperator{\honestgapi}{\mathnormal{\mu_{\honestarm} - \ \mu_i}}
\DeclareMathOperator{\honestmean}{\mu_{\honestarm}}
\DeclareMathOperator{\honestset}{\mathnormal{\arms}_{\mathcal{H}}}
\DeclareMathOperator{\armshonest}{\mathnormal{\arms}_{\mathcal{H}}}

\DeclareMathOperator{\barm}{\mathnormal{\bar{m}}}

\DeclareMathOperator{\Distup}{\mathcal{D}_{\mathnormal{r \ge \barm}}}
\DeclareMathOperator{\Distdown}{\mathcal{D}_{\mathnormal{r < \barm}}}

\DeclareMathOperator{\probdown}{\mathnormal{\Pr(r<\barm)}}
\DeclareMathOperator{\probup}{\mathnormal{\Pr(r \ge \barm)}}

\DeclareMathOperator{\meandown}{\mathnormal{\mu_{r <\barm}}}
\DeclareMathOperator{\meanup}{\mathnormal{\mu_{r \ge \barm}}}



\DeclareMathOperator{\alphaneg}{\mathnormal{\alpha}_{-}}



\newcommand{\compInfo}{\text{competition-informed}\xspace}
\newcommand{\CompInfo}{\text{Competition-informed}\xspace}
\newcommand{\CompInfoInitCap}{\text{Competition-Informed}\xspace}


\newcommand{\compamb}{\text{competition-ambivalent}\xspace}
\newcommand{\Compamb}{\text{Competition-ambivalent}\xspace}
\newcommand{\CompAmbInitCap}{\text{Competition-Ambivalent}\xspace}


\newcommand{\armsfaulty}{\mathcal{A}_{\text{faulty}}}
\newcommand{\armsnonfaulty}{\mathcal{A}_{\text{non-faulty}}}

\newcommand{\term}[1]{\ensuremath{\mathtt{#1}}\xspace}


\newenvironment{proofsketch}{%
\renewcommand{\proofname}{Proof Sketch}\proof}{\endproof}

\newenvironment{proofsketchandinterp}{%
\renewcommand{\proofname}{Proof Sketch and Interpretation of Condition \ref{cond:cond_good_revenue}}\proof}{\endproof}


\DeclareMathOperator{\armseq}{\mathcal{A}_{\text{prev}}}
\DeclareMathOperator{\armsnon}{\mathcal{A}_{\text{non-prev}}}

\DeclareMathOperator{\Seq}{\mathnormal{S}_{\text{prev}}}
\DeclareMathOperator{\Snon}{\mathnormal{S}_{\text{non-prev}}}
\DeclareMathOperator{\Snonp}{\mathnormal{S\prime}_{\text{non-prev}}}
\DeclareMathOperator{\Seqi}{\mathnormal{S}_{(\text{prev},\mathnormal{i})}}
\DeclareMathOperator{\Seqnoti}{\mathnormal{S}_{(\text{prev},\mathnormal{-i})}}


==> more_on_equilibrium.tex <==
\section{More on Equilibrium}\label{sec:more_equilibrium} 
\subsection{Best Performance is Not a Dominant Strategy}
Here we show that despite best performance being an equilibrium for performance incentivizing MAB algorithms. It cannot be a dominant strategy for an arm if we are using any sublinear MAB algorithm. 
% \subsection{Homogeneous Case:}\label{sec:homogenus_case}
% We being by showing that best performance is not a dominant strategy for any sublinear MAB algorithm.
\begin{theorem}
For any sublinear MAB algorithm, it is not a dominant strategy for an arm $i$ to follow the best performance strategy $S^*_i$ of always giving $M_i$.
\end{theorem}
\begin{proof}
Consider two arms $\{a_1,a_2\}$ with means $\mu_1,\mu_2$ such that $1> \mu_1 > \mu_2$ and $M_1=M_2=1$. Suppose arm 2 follows the strategy $S_2$ of not changing its rewards at all. Arm 1 has two strategy options $S^*_1$ that always gives $1$ and $S_1$ that just takes the reward without changing it. Then we have the following:
\begin{align*}
    u_1(S^*_1,S_2) = \E[T_1(n)-C_1(n)] = \E[T_1(n)-(1-\mu_1)T_1(n)] = \mu_1 \E[T_1(n)] \leq \mu_1 n 
\end{align*}
Also, we have 
\begin{align*}
    u_1(S_1,S_2) = \E[T_1(n)] \ge n-o(n) 
\end{align*}
Therefore, $u_1(S_1,S_2) = u_1(S^*_1,S_2) + (1-\mu_1) n -o(n)$, therefore $S^*_1$ is not a dominant strategy.  
\end{proof} 


%We will consider the strategy profile $S^*$ where all arms give a reward of 1.\SH{maximal reward?, i.e. what if $M_i \le 1$?}.



\subsection{Non-Existence of Sub-Optimal Profit Equilibria}\label{subsec:no_bad_equilb}
Here we show that there exists no approximate equilibrium for which the principal receives regret less than $\maxall$ for a linear number of rounds for the heterogeneous case with competition information. Specifically, we show that any MAB algorithm that is sharply robust and monotonic has no approximate equilibrium where a principal gains a revenue less than $P(n)=\maxall n-o(n)$. All that is required is an assumption on the number of top arms and their means as given below: 
% We give the proof for the heterogeneous case with information. Note that the same proof holds for the homogeneous case by replacing $\maxall=1$, $\armstop= \arms$, and $\bk=k$. 

\begin{condition}\label{cond:cond_good_revenue}
$\min_{i \in \armstop} (1+\meani-\maxall) > \frac{1}{\bk}$. 
\end{condition}

\begin{theorem}\label{th:sr_np_bad_equilib}
Given a MAB algorithm that satisfies sharp robustness and monotonicity, then if Condition (\ref{cond:cond_good_revenue}) is satisfied, then there exists no approximate equilibrium strategy profile $S$ such that $P(n)\leq \alpha \maxall n +o(n)$ where $\alpha <1$. 
\end{theorem}
\begin{proof}
We start with the following claim which shows that best performance is not played by an in $\armstop$.
\begin{claim}
If $P(n)\leq \alpha \maxall n$ where $\alpha <1$ for strategy profile $S=(S_1,\dots,S_k)$, then it cannot be the case that there exists an arm $i \in \armstop$ such that $S_i=\Sbesthet$.
\end{claim}
\begin{proof}
By contradiction, if that was the case, then the MAB instance would be reduced to an instance where arm $i$ can be considered as the top arm with $\toteffort{i}(n)=0$ and $\meani=\mu^*=\maxall$. Since a sharply robust algorithm always has sublinear regret (Theorem (\ref{th:sr_always_sb_regret})), then $R(n)=o(n)$ and hence $P(n)=\maxall n- R(n)=\maxall n -o(n)$ which is a contradiction. Therefore, it must be the case that $\forall i \in \armstop$, we have $S_i \neq \Sbesthet$. 
\end{proof}
Now we define $\tcal$ to be a subset of rounds such that: 
\begin{align}
\E[\sum_{t\in \tcal} \Tilde{r}_{I_t}(t)] < \maxall \E[|\tcal|]
\end{align}
then the following claim must be true: 
\begin{claim}\label{cl:tcal_size}
$\E[|\tcal|] \ge (1-\alpha) n-o(n)$.
\end{claim}
\begin{align*}
    \alpha \maxall n + o(n) & \ge P(n)=\maxall n -\E[\sum_{t\in \tcal} \Tilde{r}_{I_t}(t)]  > \maxall n- \maxall \E[|\tcal|] \\
            \iff & \alpha n + o(n) >  n- \E[|\tcal|] \\ 
            \iff &  \E[|\tcal|] > (1-\alpha) n -o(n) 
\end{align*}
Before going to the core of the proof. We also show the following helpful claim: 
\begin{claim}\label{cl:pulls_increase}
If an arm $i \in \armstop$ was to deviate from $S_i$ to $\Sbesthet$, then $\E[\totpulls{i}(n)|\Sbesthet,S_{-i}] = \E[\totpulls{i}(n)|S_i,S_{-i}] + \E[\sum_{t\in \tcal} \indic[I_t \neq i]]$. 
\end{claim}
\begin{proof}
Defining the subset of rounds $\tcal^c$ to be the complement of the set $\tcal$. Then: 
\begin{align*}
    n = \E[|\tcal^c| | \Sbesthet,S_{-i}] + \E[|\tcal| | \Sbesthet,S_{-i}]  
\end{align*}
Since arm $i \in \armstop$ has deviated to $\Sbesthet$, then we have a MAB instance with $\mu^*=\maxall$. Therefore, by the sublinear regret property of sharply robust algorithms (Theorem (\ref{th:sr_always_sb_regret})) and the definition of $\tcal$, then $\E[|\tcal| | \Sbesthet,S_{-i}]=o(n)$. Since by Claim (\ref{cl:tcal_size}), the $(1-\alpha) n-o(n)$ have to be ``distributed'' among the arms, but by the monotonicity property, we have: $\forall j \neq i: \E[\totpulls{j}(n)|\Sbesthet,S_{-i}]\leq \E[\totpulls{j}(n)|S_i,S_{-i}]$. Thus, $\E[\totpulls{i}(n)|\Sbesthet,S_{-i}] =  \E[\totpulls{i}(n)|S_i,S_{-i}] + \E[\sum_{t\in \tcal} \indic[I_t \neq i]]$. 
\end{proof}
Now for the strategy profile $S$, we divide the set of arms according to their expected number of pulls $\E[\totpulls{i}(n)]$ into three sets: 
\begin{enumerate}
    \item $\armssl$: $\forall i \in \armssl$ we have$ \ \E[\totpulls{i}(n)]=o(n)$.
    \item $\armstcal$: $\forall i \in \armstcal$ we have$ \ \E[\totpulls{i}(n)]=\Omega(n)$ and $\E[\sum_{t\in \tcal} \indic[I_t=i]]\ge \E[\totpulls{i}(n)]-o(n)$. 
    \item $\armsntcal$: $\forall i \in \armsntcal$ we have$ \ \E[\totpulls{i}(n)]=\Omega(n)$ and $\E[\sum_{t\in \tcal} \indic[I_t=i]]=\theta_i \E[\totpulls{i}(n)]+o(n)$ where $\theta_i\in[0,1)$ is a constant.
\end{enumerate}
In words, $\armssl$ has a sublinear number of pulls unlike the other two sets. Further, each arm in $\armstcal$ almost fully intersects with $\tcal$, unlike the arms in $\armsntcal$ which only partially intersect. We now do our proof by cases: 

\paragraph{Case ($\exists i \in \armstop \cap \armssl$):} This implies that $u_i(S)=o(n)$. Therefore, if $i$ deviates to $\Sbesthet$ then by Claim (\ref{cl:pulls_increase}), we have $\E[\totpulls{i}(n)|\Sbesthet,S_{-i}] = \E[\totpulls{i}(n)|S_i,S_{-i}] + \E[\sum_{t\in \tcal} \indic[I_t \neq i]]$. Further, by Claim (\ref{cl:tcal_size}) and the fact that $i \in \armssl$, then $\E[\sum_{t\in \tcal} \indic[I_t \neq i]] \ge (1-\alpha)n-o(n)$ and hence $\E[\totpulls{i}(n)|\Sbesthet,S_{-i}]\ge (1-\alpha)n-o(n)$. Therefore, $u_i(\Sbesthet,S_{-i})\ge (1-\alpha) (1+\meani-\maxall)n-o(n)$. Clearly, $\lim_{n\rightarrow \infty}\frac{u_i(\Sbesthet,S_{-i})}{u_i(S_i,S_{-i})}=\infty$ and therefore $S$ is not an equilibrium strategy profile. 

Since by the above if $\exists i \in \armstop \cap \armssl$, then we do not have an equilibrium. Therefore, we assume that all arms in $\armstop$ are distributed among $\armstcal$ or $\armsntcal$. Since $ |\armstop| = \bk$, then there must exist an arm in $i \in \armstop$ such that $\E[\sum_{t\in \tcal} \indic[I_t = i]]\leq \frac{\E[|\tcal|]}{\bk}\leq \frac{(1-\alpha)n}{\bk}-o(n)$. 


\paragraph{Case ($\exists i \in \armstop \cap \armstcal$ and $\E[\sum_{t\in \tcal} \indic[I_t = i]]\leq \frac{(1-\alpha)n-o(n)}{\bk}$):} Since $\E[\sum_{t\in \tcal} \indic[I_t=i]]\ge \E[\totpulls{i}(n)]-o(n)$, then $\E[\totpulls{i}(n)] \leq \frac{\E[|\tcal|]}{\bk}\leq \frac{(1-\alpha)n}{\bk}-o(n)$. Therefore, $u_i(S)\leq \frac{(1-\alpha)n}{\bk} -o(n)$. Now suppose, arm $i$ deviates to $\Sbesthet$, then again by Claim (\ref{cl:pulls_increase}) and definition of $\armstcal$, we have $\E[\totpulls{i}(n)|\Sbesthet,S_{-i}] = \E[\totpulls{i}(n)|S_i,S_{-i}] + \E[\sum_{t\in \tcal} \indic[I_t \neq i]]\ge \frac{(1-\alpha)n}{\bk} + \frac{\bk-1}{\bk} (1-\alpha)n - o(n) = (1-\alpha)n-o(n)$. Therefore, $u_i(\Sbesthet,S_{-i})\ge (1-\alpha) (1+\meani-\maxall) n-o(n)$. By Condition (\ref{cond:cond_good_revenue}), we have $(1+\meani-\maxall)>\frac{1}{\bk}$ and therefore we do not have an equilibrium. 

\paragraph{Case ($\exists i \in \armstop \cap \armsntcal$ and $\E[\sum_{t\in \tcal} \indic[I_t = i]]\leq \frac{(1-\alpha)n-o(n)}{\bk}$):} We have $u_i(S)\leq \E[\sum_{t\in \tcal} \indic[I_t = i]] + (1+\meani-\maxall)\E[\sum_{t\notin \tcal} \indic[I_t = i]] \leq \frac{(1-\alpha)n}{\bk}+(1+\meani-\maxall) (1-\theta_i) \E[\totpulls{i}(n)] - o(n)$. Now if $i$ deviates to $\Sbesthet$, then we have similarly by Claim (\ref{cl:pulls_increase}) and definition of $\armsntcal$, that $\E[\totpulls{i}(n)|\Sbesthet,S_{-i}] \ge (1-\alpha)n + (1-\theta_i) \E[\totpulls{i}(n)|S_i,S_{-i}] -o(n)$. Therefore, we have $u_i(\Sbesthet,S_{-i}) \ge (1-\alpha) (1+\meani-\maxall) n + (1+\meani-\maxall) (1-\theta_i) \E[\totpulls{i}(n)|S_i,S_{-i}] -o(n)$. Again, by Condition (\ref{cond:cond_good_revenue}), this implies a linear increase in the utility and therefore $S$ is not an approximate equilibrium.
\end{proof}




While the above result, shows that sharp robustness and monotonicity lead to the principal having a profit of $P(n)=\maxall n-o(n)$, we show that sharp robustness and monotonicity are not sufficient for the best performance strategy profile $\Sbest=(\Sbest_1,\dots,\Sbest_k)$ to be an approximate equilibrium. We do this by finding a constructive example as shown in the next theorem: 
\begin{theorem}
Sharp robustness is not sufficient to have $\Sbest=(S^*_1,\dots,S^*_k)$ be an approximate equilibrium.
\end{theorem}
\begin{proof}
Consider a variant of $\epsilon$-Greedy which is identical to Box (\ref{alg:eps_greedy}) in Appendix (\ref{sec:eps_greedy_PI}) except that when it exploits (line 3, with $s_t=0$) instead of choosing uniformly among the set of arms with highest empirical mean, it instead chooses the arm with the highest empirical mean and brakes ties in favor of the arm with the lowest index instead of sampling uniformly. 

Note that this variant of $\epsilon$-Greedy still satisfies sharp robustness (Theorem \ref{th:eps_greedy_sr}) as uniform sampling is never invoked in the proof. However, the FATA property is clearly not satisfied. Consider the case where $k=2$ and best performance strategy profile $S^*=(S^*_1,S^*_2)$, then it follows that $\E[T_2(n)]=\E[T^R_2(n)]$ where $T^R_2(n)$ is the number of pulls arm $2$ receives in the exploration rounds, this the case since arm $1$ would always be chosen for exploitation. It follows that $u_2(S^*_1,S^*_2)=\mu_2 \E[T^R_2(n)]$. On the other hand, if arm $2$ was to deviate to a strategy $S'_2$ where is does no improvement, then $u_2(S^*_1,S'_2)=\E[T^R_2(n)]$. It follows that $S^*=(S^*_1,S^*_2)$ is not an equilibrium since we do not have: $\lim_{n \to \infty} \frac{u_i(S^*_1, S'_2)}{u_i(S^*_1,S^*_2)} = \frac{1}{\mu_2} >1$ contradicting Definition (\ref{def:one_approx_equilib}). 
\end{proof}


\paragraph{Interpretation of Condition (\ref{cond:cond_good_revenue}) and Theorem (\ref{th:sr_np_bad_equilib}):} Essentially if the number of top arms $\bk$ is very large, then there must be a top arm that gets at most $\frac{1}{\bk}$ of the horizon. Roughly speaking, if there is a linear proportion $\alpha n$ of the horizon where the performance is not optimal (rewards of $\maxall$) and if the cost of performing at the top value which is $(\maxall-\meani)$ in expectation is relatively small as implied by the condition $1-(\maxall-\meani) > \frac{1}{\bk}$, then this arm would have the incentive to deviate to a top performance level to take the $\alpha n$ portion of the horizon. This result also implies that the principal can make sure that she always obtains optimal revenue by increasing the number of top arms (higher $\bk$) and by making the gap needed for optimal performance $(\maxall-\meani)$ small. Both of these considerations are intuitive and simple.   

%\SE{With some modification Theorem (\ref{th:sr_np_bad_equilib}) holds even when arms can steal their rewards.}  
\SE{New}
\begin{theorem}\label{th:sr_np_bad_equilib}
Given a MAB algorithm that satisfies sharp robustness, then there exists no approximate equilibrium strategy profile $S$ such that $P(n)\leq \alpha \maxall n +o(n)$ where $\alpha <1$. 
\end{theorem}
\begin{proof}
Now we define $\topt$ and $\tsubopt$ to be a subset of rounds such that: 
\begin{align}
& \E[\sum_{t\in \topt} \Tilde{r}_{I_t}(t)] = \maxall \E[|\topt|] \\
& \E[\sum_{t\in \tsubopt} \Tilde{r}_{I_t}(t)] < \maxall \E[|\tsubopt|]
\end{align}
then the following claim must be true: 
\begin{claim}\label{cl:tsubopt}
$\E[|\tsubopt|] \ge (1-\alpha) n-o(n)$.
\end{claim}
\begin{proof}
\SH{are we proving by contradiction?}
\begin{align*}
    \alpha \maxall n + o(n) & \ge P(n)=\maxall n -\E[\sum_{t\in \tsubopt} \Tilde{r}_{I_t}(t)]  > \maxall n- \maxall \E[|\tsubopt|] \\
            \iff & \alpha n + o(n) >  n- \E[|\tsubopt|] \\ 
            \iff &  \E[|\tsubopt|] > (1-\alpha) n -o(n) 
\end{align*}
Before going to the core of the proof.
\end{proof}
Under strategy profile $S$, for any arm $i$ we define the following: 
\begin{align}
& \E[\sum_{t\in \topt}  \indic[I_t=i] ] = \thetaopti{i}(S) n + o(n) \\
& \E[\sum_{t\in \tsubopt}  \indic[I_t=i] ] = \thetasubopti{i}(S) n + o(n) 
\end{align}
Further for any arm $i$ define its average rewards during the rounds when it is pulled in $\tsubopt$ by:
\begin{align}
    \avgi{i}  = \frac{\E[\sum_{I_t= i, t\in \tsubopt} \Tilde{r}_{I_t}(t)]}{\E[\sum_{t\in \tsubopt}  \indic[I_t=i] ]}
\end{align}
if $\E[\sum_{t\in \tsubopt}  \indic[I_t=i] ]=0$, then set $\avgi{i}=0$. 


\paragraph{Case 1, There exists more than one arm $i$ with $\thetasubopti{i}(S)>0$:} 
Let $i'=\argmax\limits_{i \in \armstop} \avgi{i}$ and let $i''$ be the index with the second highest $\avgi{i}$. Let $i'$ deviate from its strategy $S_i$ to $S'_i$ where for the first $\thetaopti{i}(S) n$ pulls it gives $\maxall$ and for the rest of the pulls it gives $\avgi{i'}+\epsilon$ where $\epsilon>0$ is a constant. 

By sharp robustness arm $i$ will be pulled for $\thetaopti{i}(S) n$ pulls\SH{I don't understand it}. Further, $\forall j\neq i: \thetasubopti{j}(S')=0$ \SH{Isn't there more than one such $i$?}. For $i$, the utility under $S$ is $u_i\leq (1+\meani-\maxall) \thetaopti{i} n + (1+\meani-\avgi{i}) \thetasubopti{i} n + o(n)$ whereas under $S'$ the utility is $u'_i \ge  (1+\meani-\maxall) \thetaopti{i} n + (1+\meani-\avgi{i'}-\epsilon) \E[|\tsubopt|]$. For a small enough $\epsilon$ we have $\lim\limits_{n \xrightarrow{} \infty} \frac{u'_i}{u_i}=\infty$. 

\paragraph{Case 2, There exists only one arm $i$ with $\thetasubopti{i}(S)>0$:} 
Let $j$ be the arm with $\thetasubopti{j}(S)>0$. Then consider an arm $i \in \armstop$ such that $i \neq j$. Suppose $i$ from $S_i$ deviates to $S'_i$ where for the first $\thetaopti{i}(S) n$ pulls it gives $\maxall$ and for the rest of the pulls it gives $\avgi{j}+\epsilon$ where $\epsilon>0$ is a constant. 

By sharp robustness arm $i$ will be pulled for $\thetaopti{i}(S) n$ pulls. Further, $\forall j\neq i: \thetasubopti{j}(S')=0$. For $i$, the utility under $S$ is $u_i\leq (1+\meani-\maxall) \thetaopti{i} n + (1+\meani-\avgi{i}) \thetasubopti{i} n + o(n)$ whereas under $S'$ the utility is $u'_i \ge (1+\meani-\maxall) \thetaopti{i} n + (1+\meani-\avgi{j}-\epsilon) \E[|\tsubopt|]$. For a small enough $\epsilon$ we have $\lim\limits_{n \xrightarrow{} \infty} \frac{u'_i}{u_i}=\infty$. 




\end{proof}


==> pure_sp_mech.tex <==
\section{Second-Price Auction Based Mechanism: How does it behave?}\label{sec:sp_is_fragile}
Here we consider solving the problem using a second-price auction (SP) based mechanism similar to what is done in \cite{braverman2019multiarmed}. Recall that each arm $i$ has a maximum value $M_i$ it can lift its reward to. The template of SP would be of the form shown in algorithm (\ref{alg:spa_mech}) below: 
\begin{algorithm}
(1) Pull each arm once, let $m_i$ be the value reported by arm $i$ and then pull each arm for $N_i$ rounds such that $\E[N_i]=2m_i$  \\
(2) Let $m'$ be the second highest value and $i^*$ be the arm that reported the highest value.\\
(3) Pull arm $i^*$ for the rest of the horizon and stop pulling it if it gives a reward less than $m'$. 
\caption{\textsc{Second-Price Mechanism}}\label{alg:spa_mech}
\end{algorithm}
The algorithm has two essential parts (line (2) only defines values): Line (1) is essentially bidding through performance and payment from the principle (by pulling) for truthful bidding (giving max performance). Line (3) is where the top arm is asked to perform well and is punished by not being pulled again. The lemma gives the natural dominant strategy:
\begin{lemma}\label{th:ds_spa_mech}
The dominant strategy for any arm is the following: 
\begin{itemize}
    \item Give reward $M_i$ the first time you are pulled, this means $m_i=M_i$. 
    \item Do not exert any effort in the rounds $N_i$. 
    \item If $i=i^*$, then always give reward $m'$. 
\end{itemize}
\end{lemma}
\begin{proof}
First it is clear that any arm's utility is maximized by not giving any effort for the rounds $N_i$ since the algorithm would not pull the arm more or less depending on the rewards in these rounds. Consider the case where $i \neq i^*$, then the arm's utility is clearly $u_i=u_i(m_i)=1-(m_i-\meani)+2m_i=(1+\meani) + m_i$ which is maximized by setting $m_i$ to the largest possible value, thus $m_i=M_i$. 

If $i = i^*$, then in line (3) where the arm is pulled, it can always guarantee itself one more pull by giving $m'$ and gain more utility of value $1-(m'-\meani)>0$. Therefore, the arm should always give $m'$, in the line (3) rounds. Further, its entire utility is $u_i= (1+\meani) + m_i + (n-\sum_{i \in [k]} N_i) (1-(m'-\meani))$, therefore the term is maximized by setting $m_i=M_i$. Further, if it reports $m_i <m'$, then this would make the overall utility smaller since it would no longer be selected as the top arm in line (3), thus $m_i=M_i$. 
\end{proof}

\paragraph{What if the arm spends an effort close to equilibrium effort?} Clearly, the top arm $i^*$ has to spend effort of expected value $(m'-\meani)\big(n-o(n)\big)$. But what if deviates (under-performs) for a number of rounds $\epsilon n$, this is a linear number of rounds, but I still think it's plausible and can be considered very close to the expected value of $(m'-\meani)\big(n-o(n)\big)$ since $\epsilon$ can be an arbitrarily small constant. One would still want guarantees, but clearly this would not work in the version above. So let's try this version \ref{alg:spa_mech_2} which introduces an under-performance tolerance threshold where the new additions are shown in blue and green:   

\begin{algorithm}
(1) Pull each arm once, let $m_i$ be the value reported by arm $i$ and then pull each arm for $N_i$ rounds such that $\E[N_i]=m_i$  \\
(2) Let $m'$ be the second highest value and $i^*$ be the arm that reported the highest value.\\
(3) Pull arm $i^*$ for the rest of the horizon and stop pulling it if it gives a reward less than $m'$ \textcolor{blue}{for $S$ many rounds}. \\  
(4) \textcolor{teal}{If arm $i^*$ is no longer played, then do something else.} 
\caption{\textsc{Second-Price Mechanism with Tolerance}}\label{alg:spa_mech_2}
\end{algorithm}

Let's consider the case of two arms where $M_1 > M_2$, so $i^*=i$. What should we set the value of the tolerance $S$ to? There are two possibilities: $(1): S=\alpha n$ for some constant $\alpha$, $(2):S=o(n)$. 

If $S=\alpha n$, then if $\mu_2 >\mu_1$, then it follows that the algorithm could have linear regret since even if arm $1$ can give the required value of $m'$ for the entire horizon, it would take advantage of the tolerance to reduce the cost. So we would not set $S=\alpha n$. 

If $S=o(n)$, then if arm $1$ actually deviates for some rounds $s_i=S+1=o(n)$, then arm $1$ would be blocked and the mechanism would go to line (4). Further, let's assume that $\mu_1>\mu_2$ instead keeping $M_1>M_2$ as before, what should the mechanism do in line (4)?? If it doesn't play arm $1$ again, then it doesn't have sublinear regret. The arm can play arm $2$ but that doesn't guarantee sublinear regret if $\mu_1 > M_2$? Further, even if $M_2 \ge \mu_1$, how do we incentive arm 2 to keep giving good performance? It seems simpler to instead have an algorithm that gives sublinear regret always. This failure discussion can also be made in the case of homogenus arms (same top max value). 



==> reproduce.tex <==
\section*{Reproducibility Checklist}
Below we give the answers to the reproducibility checklist for this paper. 
\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced: \textcolor{blue}{Yes}
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results:\textcolor{blue}{Yes}
    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper: \textcolor{blue}{Yes}
    \item Does this paper make theoretical contributions? \textcolor{blue}{Yes}
    \item All assumptions and restrictions are stated clearly and formally. \textcolor{blue}{Yes}
    \item All novel claims are stated formally (e.g., in theorem statements). \textcolor{blue}{Yes}
    \item Proofs of all novel claims are included. \textcolor{blue}{Yes}
    \item Proof sketches or intuitions are given for complex and/or novel results. \textcolor{blue}{Yes}
    \item Appropriate citations to theoretical tools used are given. \textcolor{blue}{Yes}
    \item All theoretical claims are demonstrated empirically to hold. \textcolor{blue}{No}
    \item All experimental code used to eliminate or disprove claims is included. \textcolor{blue}{NA}
    \item Does this paper rely on one or more datasets? \textcolor{blue}{No}
    \item Does this paper include computational experiments? \textcolor{blue}{No}
\end{itemize}

% \section*{Broader Impact Statement} 
% The practical deployment of machine learning algorithms can clearly have consequences on the welfare of individuals. Therefore, stakeholders should be consulted and possible negative harms should be thought out. We do not see any negative implications of our work or clear ethical consideration. However, our work has been from the perspective of the principal who is concerned with the total revenue obtained. Although, our algorithms do not degrade the agents' utilities (cause harm) in a clear or direct manner, we have not provided fairness guarantees for the agents. 
% Therefore, a possible direction and consideration for future work is to augment our algorithms with agent-focused fairness and welfare guarantees. 

==> ucb_properties.tex <==
\section{UCB is Performance Incentivizing}\label{app:UCB}
Theorem \ref{th:UCB1_robust} proves that UCB is sharply adaptive here we show that it satisfies monotinicity (Theorem \ref{th:ucbmono}) and FATA (Theorem \ref{th:ucbfata}) as well. For completeness, the algorithm block below shows the full pseudo-code for UCB\SE{in the main paper}. 
% \begin{algorithm}
% Play each arm once for the first $k$ rounds.\\
% In a given round $t>k$:  \\
% \ \ Pull arm $i$ with highest $UCB_i(t-1)=\hat{\mu}_i(t-1)+\sqrt{\frac{2 \ln(n)}{\totpulls{i}(t-1)}}$ (breaking ties arbitrarily) 
% \caption{\textsc{UCB}}\label{alg:ucb}
% \end{algorithm}


